On Fourier algebra of a hypergroup constructed from a conditional expectation on a locally compact group

We prove that the Fourier space of a hypergroup constructed from a conditional expectation on a locally compact group has a Banach algebra structure.

==> jinfo.tex <==
\jvolume{23}
\jyear{2017}
\jnumber{1}

